Successive Embedding and Classification Loss for Aerial Image Classification

Deep neural networks can be effective means to automatically classify aerial images but is easy to overfit to the training data. It is critical for trained neural networks to be robust to variations that exist between training and test environments. To address the overfitting problem in aerial image classification, we consider the neural network as successive transformations of an input image into embedded feature representations and ultimately into a semantic class label, and train neural networks to optimize image representations in the embedded space in addition to optimizing the final classification score. We demonstrate that networks trained with this dual embedding and classification loss outperform networks with classification loss only. %We also study placing the embedding loss on different network layers. We also find that moving the embedding loss from commonly-used feature space to the classifier space, which is the space just before softmax nonlinearization, leads to the best classification performance for aerial images. Visualizations of the network's embedded representations reveal that the embedding loss encourages greater separation between target class clusters for both training and testing partitions of two aerial image classification benchmark datasets, MSTAR and AID. Our code is publicly available on GitHub.

==> 6biography.tex <==

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/JiayunW.jpg}}]{Jiayun Wang} is currently pursing the Ph.D. degree in Vision Science from University of California, Berkeley. He is also a graduate student researcher at the International Computer Science Institute. He received his B.E. degree in Electronic Engineering from Xi'an Jiaotong University, China. His research interests include computer vision and pattern recognition, with a focus
on target recognition, image classification and generative models.
\end{IEEEbiography}
% if you will not have a photo at all:
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,trim={0 0 .25in 0},clip,keepaspectratio]{img/virtue.jpg}}]{Patrick Virtue} is a Ph.D. candidate in Electrical Engineering and Computer Sciences at the University of California, Berkeley, specializing in deep learning, computer vision, and image processing. He has applied his work to a range of applications from medical imaging to  military target detection. He earned his B.S. degree in Computer Science Engineering at the University of Notre Dame. Prior to graduate school, he researched and developed medical image applications as a software engineer at GE Healthcare.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/syu.jpg}}]{Stella X. Yu} received her doctorate from the School of Computer Science at Carnegie Mellon University, where she studied robotics at the Robotics Institute and vision science at the Center for the Neural Basis of Cognition.  She is the director of the Vision Group at the International Computer Science Institute, and a Senior Fellow at the Berkeley Institute for Data Science, UC Berkeley.  Dr. Yu is interested in understanding visual perception from multiple perspectives: human vision, computer vision, robotic vision, and artistic vision.
\end{IEEEbiography}


==> Deprecated_1Intro_merged.tex <==
\section{Introduction}

Synthetic aperture radar (SAR) captures images of objects that are suitable for target classification, reconnaissance and surveillance, regardless of the day-and-night conditions.
Target recognition in SAR images has many potential applications in military and homeland security, such as friend and foe identification, battlefield
surveillance, and disaster relief.

Automatic target recognition (ATR) for SAR images often proceeds in two stages: detection and classification.
At the detection stage, candidate target patches are extracted from  SAR images; they may include not only targets of interest, but also false alarm clutter such as trees, cars, buildings, etc. 
These detected image regions, so called \textit{chips}, are then sent to the classification stage, where a classification algorithm predicts the target class of each chip.  In this work, we focus on improving the chip classification accuracy.

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{img/bar.pdf}
\caption{Our algorithm aims to  learn the discriminate feature of input SAR chips for improving SAR target classification performance. We learn the discriminative feature by adopting both embedding loss and  classification loss, and achieve improved classification and outlier rejection performance. We also find that applying embedding loss on classifier space (solid line) has better performance than on other space (dashed line). Additionally, we evaluate the performance of different types of embedding loss, and find that center loss has better overall performance. }
 \label{overview}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{img/intro_2.pdf}
\caption{Our algorithm aims to  learn the discriminate feature of input SAR chips for improving SAR target classification performance. We learn the discriminative feature by adopting both embedding loss and  classification loss, and achieve improved classification and outlier rejection performance. We also find that applying embedding loss on classifier space (solid line) has better performance than on other space (dashed line). Additionally, we evaluate the performance of different types of embedding loss, and find that center loss has better overall performance. }
 \label{overview}
\end{figure}




\def\widthA{0.47}
\def\widthB{0}
\def\widthC{0.33}

\begin{figure*}[ht]
\centering
\tb{@{}ccc@{}}{0.5}{
{} & {Contrastive loss} & Contrastive loss \\  [0.75ex]
{ Softmax Loss} & {on Feature Space} & on Classifier Space \\

	\imw__{orth_base}{\widthC}{\footnotesize } &
		\imw__{orth_fc6}{\widthC}{\footnotesize } &
	\imw__{orth_fc7}{\widthC}{\footnotesize } 

}
\caption{Orthogonal projection visualization of classfier space on two-target axes (BTR60 and BTR70). The table on the lower right shows the confusion matrix of the two targets. Single classifier: Only classfication loss is applied. The big intra-class variance of the two classes (BTR60 and BTR70) leads to inter-class overlapping and confusion between them. With dual contrastive loss applied on feature space, the intra-class variance decreases. However, the inter-class overlapping between BTR60 and BTR70 still exists. Moving the contrastive loss to the classifier space, the intra-class variance is relatively small, leading to less inter-class confusion. The classification performance is improved by learning the discriminative feature.}
\label{fig:ortho}
\end{figure*}

% Recently, deep learning methods have used for SAR target recognition, integrating feature extraction and classification into a single trained neural network \cite{nisar} \cite{chenini} ~\cite{morgan} \cite{wangsar} \cite{ding} \cite{chen} \cite{wagnerSAR} \cite{linSAR}.

Traditional SAR target classification methods rely on extracting informative features and applying powerful classifiers.
Various features have been explored, including raw pixel intensity \cite{chen9}, magnitudes of the 2-D DFT coefficients \cite{chen10}, and a transform of the SAR image into polar coordinates followed by PCA compression \cite{chen3}. Popular classifiers include support vector machines \cite{chen9}, radial basis function networks \cite{chen10} and nearest neighbor \cite{chen3}.

In recent years, the deep learning based methods have become increasingly popular in image classification. In 2012, Krizhevsky \etal demonstrated the effectiveness of deep learning on large-scale problems by using convolutional neural networks (CNNs) to attain superior image classification accuracy on the ImageNet Large Scale Visual Recognition Challenge (ILSVRC) data set \cite{ding8}.
%Simonyan \etal \cite{ding10} introduced a 22-layer CNN for classification and 16-layer and 19-layer deep CNNs for large image recognition.
In 2013, Ni and Xu applied deep learning to train a sparse autoencoder network to learn a feature representation that they used to train a linear softmax regression classifier \cite{nisar}. In 2014, Chen and Wang combined feature learning and classification by training an end-to-end CNN to classify SAR images \cite{chenini}. Chen \etal then proposed an all-convolutional network (A-ConvNets), which outperformed equivalent CNNs that included fully connected layers \cite{chen}. 
In order to address the challenges of real-world SAR images, Ding \etal augmented the Moving and Stationary Target Acquisition and Recognition (MSTAR) public dataset  \cite{chen7} with random translation and with random noise to create a more challenging test environment for their CNN SAR classification experiments \cite{ding}.
To address the limited availability of SAR training data, Lin \etal used a deep convolutional highway unit network trained with a reduced dataset \cite{linSAR}.
% Wagner \etal  presented a new network architecture for SAR target classification, which has a more flexible structure and reduced training time.

Despite the appreciable achievements that these deep models achieved in SAR target recognition, the complexity of the real-world SAR images still cause challenging differences between the training scenario and different test scenarios, including variations in depression angle, SAR sensors, landscape, target articulation, and target configuration. Using basic classification convolution neural networks, the training accuracy can reach 100\%, while the test accuracy is below 90\% \cite{ding}.

%Classification loss is not enough for SAR target classification. To address the overfitting problem, we proposed to use both classification loss and embedding loss for learning the discriminative feature and higher performance classifier. Recent work shows the success of using both loss functions to improve the performance in re-identification tasks. 

To address the aforementioned overfitting problems, trained networks should be more discriminative, namely the learned representations should have small intra-class variation while maintaining large inter-class variation. Using the classification loss is not enough for learning a discriminative classifier. We seek to further improve the SAR target classification accuracy by applying embedding loss, in addition to the classification loss. \textit{Contrastive loss} is a representative of embedding loss that seeks to reduce the distance between a pair of training points if they have the same class, and increase the distance if the two points belong to different classes. Chopra \etal  proposed the contrastive loss to train a Siamese network to learn a similarity metric for face images \cite{chopra2005learning}. %Siamese networks were first proposed by Bromley \etal for signature verification \cite{bromley1994signature}.

%In addition to working as a similarly metric, contrastive loss can also be used for classification.
Previous work demonstrates the success of using both classification loss and embedding loss in re-identification tasks, which aims to re-identify unknown class (person) in test phase.
Sun \etal  first demonstrated that the contrastive loss can also act as an embedding loss for re-identification tasks, since it can decrease intra-class variance and increase inter-class differences, as well as being compatible with classification loss (softmax cross-entropy loss) \cite{sun2014deep}.
Using both classification loss and contrastive loss as supervision, their network was able to learn discriminative facial features with reduced intra-personal variations and enlarged inter-personal differences. The discriminative feature helps improve the performance of the re-identification tasks.

In addition to contrastive loss, some work used other embedding loss for re-identification. For example, Wen \etal~\cite{wen2016discriminative} used \textit{center loss} to simultaneously learn a center for deep features of each class and penalizes the distances between the deep features and their corresponding class centers. Other possible embedding loss functions include triplet loss \cite{schroff2015facenet}, point-to-set (P2S) loss \cite{p2s} and adaptive margin loss \cite{adamargin}. 

The dual embedding and classification loss was only used for re-identification tasks before, and demonstrate the potential of anti-overfitting and generalization to unseen instances. We first use the dual loss for classification. Our experiments demonstrate that by applying dual loss for SAR target classification, the learned feature is more discriminative, and the target classification   and outlier rejection performance are improved.

On which layer to apply the embedding loss, we demonstrate that applying it on the classifier space is more impactful.
All of the previous dual loss work applied the embedding loss to the feature space. %\cite{sun2014deep}~\cite{wen2016discriminative}~\cite{zheng2016discriminatively}
We propose moving the embedding loss from the feature space to the classifier space for SAR target classification, as depicted in Figure \ref{overview}. The rationales behind this include: 1) good feature representation is important, but it is ultimately the classifier space that we want to be discriminative; 2) a much smaller dimensional space can provide a more impactful distance metric; 3) applying the embedding loss to the classifier space can also lead to a discriminative feature space via back-propagation. The orthogonal projection visualization of learned classifier space (Fig. \ref{fig:ortho}) showed that applying dual embedding loss on classifier space leads to more discriminative feature and less inter-class confusion.

We compare different types of embedding loss, and find that contrastive loss has better overall performance. We evaluate our discriminative classification methods with two embedding loss functions, contrastive loss and center loss, on the MSTAR dataset \cite{chen7}. The experimental results show that including a embedding loss on the feature space improves SAR target classification accuracy from 91\% to 92\%-96\% over previous deep learning methods. Additionally, we demonstrate that moving embedding loss from feature space to classifier space further improves the accuracy from 92\%-96\% to 98\%. Although the two embedding loss performs equally well on classification, the contrastive loss performs better on outlier rejection.

We summarize the main components and advantages of our methods as follows:
\begin{itemize}
  \item
  We demonstrate that the classification loss is not enough.  We add the embedding loss to train the deep convolutional neural network, in order to learn a discriminative feature and improve SAR target classification accuracy.
   %We use Siamese network architecture, together with our contrastive and softmax dual loss, to utilize the information of matched and mismatched class. Compared with the existing one-path network architecture, our network can greatly enhance the performance of the state-of-the-art method by learning a discriminative  distribution of different image pairs in the feature space.
  \item
  We investigate which layer to apply the embedding loss.
  %We move the embedding loss from feature space to classifier space.
  The classification accuracy is better and the learned classifier space is more discriminative if the embedding loss is applied on classifier space. 
  \item
  We compare different types of embedding loss. We find that contrastive loss has better overall performance.
  %We conduct experiments to evaluate various aspects of the proposed method on the benchmark dataset MSTAR. The results outperform the previous SAR classification methods. %The visualization of the learned feature space is discriminative.
  
\end{itemize}

%The rest of the paper is organized as follows: Section \ref{sec:method} 

==> points.tex <==

%Points to make


%1) Siamese vs single classifier
%2) dual loss 
%3)  
%* compare adding contrastive loss on fc6 and fc7 
%* compare with new center loss
%4) improvement on seen and unseen instances
%5) visualization of feature tSNE 
